Searching for Winograd-aware Quantized Networks

Lightweight architectural designs of Convolutional Neural Networks (CNNs) together with quantization have paved the way for the deployment of demanding computer vision applications on mobile devices. Parallel to this, alternative formulations to the convolution operation such as FFT, Strassen and Winograd, have been adapted for use in CNNs offering further speedups. Winograd convolutions are the fastest known algorithm for spatially small convolutions, but exploiting their full potential comes with the burden of numerical error, rendering them unusable in quantized contexts. In this work we propose a Winograd-aware formulation of convolution layers which exposes the numerical inaccuracies introduced by the Winograd transformations to the learning of the model parameters, enabling the design of competitive quantized models without impacting model size. We also address the source of the numerical error and propose a relaxation on the form of the transformation matrices, resulting in up to 10% higher classification accuracy on CIFAR-10. Finally, we propose wiNAS, a neural architecture search (NAS) framework that jointly optimizes a given macro-architecture for accuracy and latency leveraging Winograd-aware layers. A Winograd-aware ResNet-18 optimized with wiNAS for CIFAR-10 results in 2.66x speedup compared to im2row, one of the most widely used optimized convolution implementations, with no loss in accuracy.

==> latency.tex <==
% \section{Building Winograd Latency Models}
\section{A Study on Winograd's Impact on Latency}
\label{latencymodels}
\todo{this section feels like a bit of an orphan, as it's essentially results and results discussion.  Does it make sense to move this to a subsection of the results?}

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\linewidth]{media/benchmarkLight.pdf}
    \vspace{-7mm}
    \caption{Latencies (expressed in milliseconds) of convolving increasingly larger input tensors in the width/height dimensions (y axis) and in depth (x axis). We compare the time needed for \textit{im2row} and each of the Winograd configurations with 32-bit arithmetic. We show that (1) \textit{im2row} is the optimal algorithm for the input layer to a network, (2) the choice between F4 and F6 should be done based on the output's width/height and, (3) the choice of Winograd configuration shouldn't change based on $inCh\rightarrow outCh$. The measurements were taking using Arm's Compute Library Winograd implementation of \citet{maji2019efficient} on a HiKey 960 with A73 and A53 cores.}
    \label{fig:latency}
\end{figure*}


The speedups associated to the use of Winograd convolutions often only account for the point-wise stage while assuming negligible costs for the input, weights and output transformations. Furthermore, these also assume that the larger the input patch, \textit{d}, the larger the speedup compared to normal convolutions. However, although these assumptions are true for large tensors, they are not necessarily true when working with tensors of the sizes often found in CNNs for image classification or object detection.

In this section we present our observations after performing a dense benchmark of multiple Winograd configurations while varying input's size and input and output channels, $inCh\rightarrow outCh$. %We show that the dimensions of the input image plays a decisive role on the choice of $d$'s dimensions. We also show that the costs of transforming the input path $d$ could be up to $\sim30\%$ of the total.
Because ultimately the use of alternative convolution implementations is to speedup inference on a target device, the parameterization of such algorithms (e.g. tile size) should be done based on the capabilities of such device to exploit these. 

% For our study we chose Arm's A73 and A53 cores running of a Huawei HiKey 960 development board with big.LITTLE CPU architecture. These cores are the building blocks of Qualcomm's Snapdragon 835 mobile platform and are present in Samsung's Galaxy S8 and Google's Pixel 2, among others. We found these Cortex-A cores to be good candidates for validating the speedups that are achievable with Winograd convolutions in today's off-the-shelve hardware. 

For our benchmark, we compared \textit{im2row} against F2, F4 and F6 Winograd convolutions. We also measure the impact on latency of applying the Winograd transformations. Figure \ref{fig:latency} shows a portion of the obtained latency measurements for our benchmark using 32-bit precision. An almost identical pattern appears when using 8-bit arithmetic. Our observations can be summarized in three points:

\begin{itemize}
    \item \textbf{Input layers do not benefit from Winograd.} This is primarily because the matrices in the element-wise stage are not large enough to compensate for the costs of transforming the input and output patches. These transformation costs represent a 45\%, 51\% and 61\% of the total costs for F2, F4 and F6 respectively given a RGB $32\times32$ input expanded to 32 channels. If it wasn't for these costs, both F4 and F6 would be lower in latency than \textit{im2row}. Similar ratios can be observed for other input sizes.
    \item\textbf{Optimal $\mathbf{m}$ is a function of input's width and height} and not of the layer's $inCh\rightarrow outCh$. For an input with sufficient number of channels, e.g. 32 channels and up, we observe a consistent pattern alternating between F4 and F6 as the channel dimension of the output increase. This alternation comes as a result of the impossibility of subdividing the input into an integer number of $(m+r-1)\times(m+r-1)$ patches and therefore having to waste calculations when operating on the input's edges. This pattern is invariant to different $inCh\rightarrow outCh$ configurations and fades away as input's dimensions exceed $40\times40$, point at which F6 consistently becomes the fastest configuration.
    \item \textbf{Input/Output transforms are costly.} Excluding inputs with very few channels, the cost of performing the transformations to/from the Winograd domain can exceed 25\% of the overall costs. This is something to take into account when considering the choice of Winograd over other convolution algorithms. %as this could represent around a 25\% of the total costs. 
\end{itemize}

% \hl{explain how models are built}

We refer the reader to~\ref{benchmarks} for a detailed description of the setup for this experiment and to the Appendix for a more results from our benchmark.
